Investigating Continual Pretraining in Large Language Models: Insights and Implications

Continual learning (CL) in large language models (LLMs) is an evolving domain that focuses on developing efficient and sustainable training strategies to adapt models to emerging knowledge and achieve robustness in dynamic environments. Our primary emphasis is on continual domain-adaptive pretraining, a process designed to equip LLMs with the ability to integrate new information from various domains while retaining previously learned knowledge. Since existing works concentrate mostly on continual fine-tuning for a limited selection of downstream tasks or training domains, we introduce a new benchmark designed to measure the adaptability of LLMs to changing pretraining data landscapes. We further examine the impact of model size on learning efficacy and forgetting, as well as how the progression and similarity of emerging domains affect the knowledge transfer within these models. Our findings uncover several key insights: (i) continual pretraining consistently improves <1.5B models studied in this work and is also superior to domain adaptation, (ii) larger models always achieve better perplexity than smaller ones when continually pretrained on the same corpus, (iii) smaller models are particularly sensitive to continual pretraining, showing the most significant rates of both learning and forgetting, (iv) continual pretraining boosts downstream task performance of GPT-2 family, (v) continual pretraining enables LLMs to specialize better when the sequence of domains shows semantic similarity while randomizing training domains leads to better transfer and final performance otherwise. We posit that our research establishes a new benchmark for CL in LLMs, providing a more realistic evaluation of knowledge retention and transfer across diverse domains.

==> 00_updates.tex <==
General updates:
- tailor the writing to clearly express (1) this is a CL work, has different objectives/scale from LLM works, (2) only a handful of CL works have our scale (give concrete numbers)
- albeit standard metrics in CL, report Anytime Perplexity (AP) and Average Anytime Perplexity (AAP):
AP_t = 1/t \sum_{i=1}^t p_{i,t} # checkpoint t, evaluated at all prev. domains
AAP = 1/T \sum_{t=1}^T AA_t # average of AAP
- reviewers tend to find results expected and reject. hence, authors should stress the unpredictability of results and make reader think about the counterfactual


1) The paper mentions that continual pretraining may not benefit models like Llama2-7B, trained on a wide and diverse corpus. However, the authors do not explore whether continual pretraining is beneficial for models trained on a corpus of data from what domains and at what scale.
------> mention that Llama data is not available, hence we cannot perform the same analysis for llama


(2) Using zero-shot perplexity and pretraining perplexity as primary evaluation metrics, while valid, may not fully capture the model's performance in real-world applications. The primary evaluation metrics used are zero-shot perplexity and pretraining perplexity, which may not fully capture the model's performance in real-world applications. Are there additional, more practical metrics that could better assess the model's utility in real-world scenarios? Can the authors incorporate user-centric metrics or task-specific accuracy measures to evaluate the model's performance comprehensively?
----------> in cl, people focus on understanding transfer/forgetting. in standard CL scenarios, they measure classification accuracy as it's their task. therefore, we measure perplexity. but because people care about downstream performances, we do that analysis as well.


(3) The findings indicate that the impact of continual pretraining varies significantly with model size. Larger models benefit more from continual pretraining, while smaller models exhibit more significant performance fluctuations, including gains and losses. What specific mechanisms cause larger models to perform more consistently and benefit more from continual pretraining compared to smaller models? Can the authors discuss potential strategies to mitigate the performance fluctuations observed in smaller models? Can specific techniques or adjustments help smaller models achieve more stable improvements?
----------> this is the first work analyzing transfer properties. it would be super interesting to combine this with knowledge preservation techniques but we are not particularly interested in it.


(4) In the key findings summarized in lines 132-141, findings (i) and (ii) are almost the same, both describing the impact of model size on pretraining. However, what is the impact? Is a larger model better? The results on LLaMa2-7B do not support this claim.
----------> change as follows: (i) CL may not be even necessary. (ii) small models are positively/negatively influenced the most.


(5) I think it is less meaningful to compute forward/backward transfer when the task orders are different, as shown in Figures 2 and 3.
----------> standard practice in CL is class-incremental, where classes have nothing in common. LLM counterpart of it is random-order. we also consider similar order as it may have interesting benefits/downsides (this is an analysis paper)


(6) I also find no clear conclusion on whether we should use a similar or random task order in continual pretraining.
----------> suggest a clear recipe


(7) Finally, finding iv (aka fine-tuning performance on standard benchmarks is indeed influenced by continual pretraining domains) is trivial and has been validated by prior studies.
----------> state that we're the first to do CL + benchmarking!


(8) In practical usage, we only focus on the average perplexity across all domains after continual pretraining, i.e., the metric "Last Checkpoint" in Table 2.
-----------> cite papers that use anytime accuracy and average anytime accuracy


(9) But why does the test perplexity of the Last Checkpoint get even worse after continual pretraining on LLaMa-2 7B and show little improvement on GPT-small, medium, and large (under M2D2 similar setting)?
------------> explain this better!


(10)  the metric "Continual Pretraining" in Table 2 (defined in line 281) only evaluates on the t-th domain after learning on the t-th domain. However, this metric does not correspond to the same checkpoint and has no practical meaning. In other words, we cannot obtain a model with the test perplexity of "Continual Pretraining" because this metric is the average (probably best) test perplexity on different domains corresponding to different checkpoints.
-----------> I'm not sure what this means but seems to require re-writing...


(11) the result on LLaMa-2 7B is also weird ("Pretraining" is much worse than "zero-shot"). I think the learning rate may be an important factor.
-----------> Include Firat's figure on lr vs perplexity


(12) Lines 17-22 state that "To this end, we introduce a new benchmark designed to measure the adaptability of LLMs to these evolving data environments, offering a comprehensive framework for evaluation." However, I am confused about what the "new benchmark" refers to.
-----------> clarify this: we propose a new way evaluation technique, did not collect new data


(13) One concern about this setup is that the corpus may have been used in the original pretraining stage.
-----------> we know for sure that this is not the case for GPT2. For Llama, it may be very well the case but it's fine, many models have closed training data and in practice one may do continual learning on the data seen during general pretraining.


(14) The writing of the paper needs improvement. For example, Line 286-287, "Our only positive forward transfer finding follows this ..." is weird; Table 2 caption, words like "This table shows" are not necessary.
-----------> correct this

==> 7_extended_related_work.tex <==

\section{Extended related work}

\subsection{Quickly read these and add below if necessary}
\begin{itemize}
    \item Don’t Stop Pretraining: Adapt Language Models to Domains and Tasks
    \item EFFECT OF MODEL AND PRETRAINING SCALE ON CATASTROPHIC FORGETTING IN NEURAL NETWORKS
    \item UNDERSTANDING CATASTROPHIC FORGETTING IN LANGUAGE MODELS VIA IMPLICIT INFERENCE
    \item TemporalWiki: A Lifelong Benchmark for Training and Evaluating Ever-Evolving Language Models
    \item Continual Mixed-Language Pretraining for Extremely Low-Resource Neural Machine Translation
    \item CONTINUAL LEARNING WITH FOUNDATION MODELS: AN EMPIRICAL STUDY OF LATENT REPLAY
\end{itemize}

\subsection{Continual learning and transfer}
\begin{itemize}
    \item \citet{ke2022continual} introduce a soft-masking mechanism to gradient in the context of continual domain-adaptive pretraining (DAP), or adapting an LLM to a sequence of unlabeled domain corpora. More specifically, the soft-masking mechanism computes the importance of the attention heads and neurons for general or domain knowledge and soft-mask them based on their importance values to control the backward gradient flow. Typically, the importance of a unit is defined by the gradient wrt that unit; however, here as a proxy, they use model robustness (how much the output changes when that unit is dropped out). They further propose a novel proxy to preserve the general knowledge in the original LLM and contrast the representations of the previously learned domain knowledge and the knowledge from the current full network. They consider a handful of training domains and downstream classification sets.
    \item \citet{wu2021pretrained} thoroughly compare the continual learning performance over the combination of 5 pretrained LLMs (ALBERT, BERT, GPT2, RoBERTa, XL-NET) and 4 CL approaches (rehearsal, regularization, dynamic architectures, mixed) on 3 benchmarks in 2 typical incremental settings. Their baselines are (i) CLINC150, an intent classification dataset with 150 classes and 100 instances per class (ii) Maven, a long-tailed event detection dataset with 163 classes, each of which is labeled at least 15 instances and (iii) WebRED, a long-tailed relation classification dataset with 243 classes, each of which is labeled with at least 15 instances. They randomly split each dataset into disjoint tasks, and each tasks contains 10 classes. Their findings show that among all LLMs, BERT is the most robust and that among all CL methods, those based on experience replay are the most performant. They also show intermediate layer representations are less prone to forgetting while the last layer (classification head) losses its calibration.
    \item \citet{hsieh2023distilling} extract LLM rationales (in the form of question and chain-of-thought answers) as supervision for training small models, called distillation step-by-step Compared to both finetuning and distillation, their mechanism achieves better performance with much fewer labeled/unlabeled training examples. 
    \item \citet{fisch2023towards} introduce a benchmark of task sequences that potentially lead to positive and negative transfer. They further propose a simple strategy for robust forward transfer, which aims to pick the checkpoint with the biggest positive knowledge transfer among all past task checkpoints.
    \item \citet{chen2023lifelong} studied lifelong learning from a sequence of online pretraining corpus distributions based on a progressively growing mixture-of-experts (MoE) architecture introduced in \citet{du2022glam}. Then freeze old experts and optimize only the newly added experts (which are initialized from old ones), ensure that only two experts are activated (hence the compute is almost fixed over time), and regularize new experts and gatings by distilling knowledge from old (frozen) experts. Their lifelong pretraining dataset contains three distributions (webpages, non-English corpus, social media conversations), a total of appr. 700B tokens.
    \item \citet{jin2021lifelong} continually pretrain LLMs over a domain-incremental research paper stream and a chronologically-ordered tweet stream with different continual learning algorithms. They show distillation-based approaches to be most effective in retaining downstream performance in earlier domains. Their dataset consists of four research areas (biomedical, computer science, material science, and physics) filtered from the S2ORC dataset.
    \item In \citet{qin2022elle}, the authors propose efficient lifelong pretraining for emerging data (ELLE), where they expand a network during learning and include domain identifying prompts during pretraining to prime the PLM which kind of knowledge it is learning. Network extension is done by adding neurons and manipulating the architecture (by simple arithmetic operations on the parameters) so that the expanded network gives the same outputs as the original one.
    \item \citet{gupta2023continual} study how to re-increase a small learning rate (aka \emph{warm-up}), which might be necessary to alleviate forgetting in continual LLM pretraining (on the Pile dataset). They also show continual pretraining with the latest pretrained checkpoint improves downstream performance (loss on a separate test, the SlimPajama dataset). In other words, selecting earlier checkpoints decreases performance, which contradicts with \citet{fisch2023towards}. This discrepancy might be because \citet{fisch2023towards} consider a domain-incremental setup while \citet{gupta2023continual} do not.
    \item \citet{razdaibiedina2023progressive} introduce progressive prompts for continual learning, where a fixed number of tokens, or prompts, are learned for each new task. They learn a separate prompt for each incoming task and concatenate the new prompt with previously learned ones. During training, only the parameters corresponding to the current prompt are learned (i.e., the old prompt and LLM parameters are frozen). 
\end{itemize}


\subsection{Fine-tuning and domain adaptation}
\begin{itemize}
    \item \citet{hu2023meta} claim that online fine-tuning does not sufficiently attend to important information, that is, the gradient signal from important tokens representing factual information is drowned out by the gradient from inherently noisy tokens. For this, they meta-train a small model to re-weight the language modeling loss for each token during online fine-tuning, in the context of out-of-date question-answering.
    \item \citet{gong2022continual} investigate continual pretraining of LLMs to improve their understanding of math problems, which is rather closer to domain adaptation in that the authors do not discuss knowledge transfer but only downstream performance.
    \item \citet{Lin2023SpecialityVG} has shown that both VLMs and LLMs tend to forget their generality due to fine-tuning to gain specialty for a specific task, and the forgetting in LLMs is influenced by the conceptual distance between a fine-tuning task and other tasks. This can be mitigated using L1 or L2 weight regularization or knowledge distillation during fine-tuning, and WiSE-FT balances pretrained generality and fine-tuned specialty the best.
    \item In \citet{mukhoti2023fine}, the authors prevent ``concept forgetting'', defined as the disability to recognize previously learned concepts that lie outside of the fine-tuning domain, by an additional loss term that preserves the features of the original foundation model during fine-tuning. 
\end{itemize}

\subsection{Additional papers}
\begin{itemize}
    \item Foundation models are shown to be highly robust against distribution shifts. Yet, the accuracy of a fine-tuned model on a shifted dataset is usually lower than the original model when tested \citep{radford2021learning}.
    \item To address this, \citet{wortsman2022robust} linearly interpolates between the original zero-shot and fine-tuned models, referred to as ``weight-space ensembling for fine-tuning (WiSE-FT)'', which substantially improves accuracy under distribution shifts while maintaining high performance on the target distribution.
\end{itemize}




==> __evaluation_setup.tex <==

\section{Evaluation setup}
This section describes our evaluation framework, where
we first set up the basic notation and subsequently specify the varied factors.
In all experiments, we start from an already pre-trained model and continue pre-training it for one epoch on all training domains subsampled from M2D2 (see the respective paragraph for dataset details).
As usual, training objectives for causal/masked language models are the next/masked token prediction likelihood.
After completing training on a domain, we checkpoint the models and compute the test perplexity on all previous domains as well as the current domain.
Please see Table~\ref{tab:notation} for the notation used in the rest of this section.

% \begin{figure}
%     \centering
%     \includegraphics[width=.49\linewidth] {figs/descriptive/cos_sim.png}
%     \includegraphics[width=.49\linewidth]{figs/descriptive/TSNEvisualization.png}
%     \caption{L1 domain similarities}
%     \label{fig:dom-sim}
% \end{figure}

\begin{figure}
  \begin{subfigure}[c]{.56\linewidth}
    \centering
    \includegraphics[width=\linewidth]{figs/descriptive/cos_sim.png}
  \end{subfigure}\hfill
  \begin{tabular}[c]{@{}c@{}}
    \begin{subfigure}[c]{.44\linewidth}
      \centering
      \includegraphics[width=\linewidth]{figs/descriptive/TSNEvisualization.png}
    \end{subfigure}\\
    \noalign{\bigskip}%
    \begin{subfigure}[c]{.44\linewidth}
      \centering
      \includegraphics[width=\linewidth,page=2]{figs/descriptive/tr_stats.png}
    \end{subfigure}
  \end{tabular}
  \caption
    {%
      Properties of our L1 training domains. \textit{(Left)} Cross-similarity matrix between training domains. For reference, we include general text in the last row/column \caca{[beyza?]}. The two big square blocks along the diagonal correspond to Wiki and S2ORC portions, respectively. \textit{(Top-right)} TSNE embeddings of \robertal activations of L1 domains \caca{[beyza?]}. Wiki domains and natural sciences are clustered near the bottom right corner and on the left, respectively. \textit{(Bottom-right)} The number of L2 domains (red) and the length \caca{[to be discussed with beyza]} of training data (blue) for each L1 domain. These together reflect the highly imbalanced nature of our data. The grey background highlights the Wiki portion. %
      \label{fig:dom-sim}%
    }
\end{figure}



\begin{table}[t!]
    \centering
    \caption{A summary of the quantities measured in our experiments}
    \label{tab:notation}
    \begin{tabular}{l|l}
    \toprule
    \textsc{Notation} & \textsc{Description} \\
    \toprule
    $D=166$ & Number of fine-grained L2 domains \\ \midrule
    $B=20$ & Number of coarse-grained L1 domains \\ \midrule
    $p_n^d$ & Perplexity of the $d$'th checkpoint computed on $n$'th domain \\ \midrule
    $z_d$ & Zero-shot perplexity a model computed on $d$'th domain (no training) \\ \midrule
    $f_d$ & Fine-tuning perplexity (training and testing a model on $d$'th domain) \\ \midrule \midrule
    $\zs=\tfrac{1}{D}\sum_d z_d$ & Average zero-shot performance \\ \midrule
    $\ft=\tfrac{1}{D}\sum_d f_d$ & Average fine-tuning performance \\ \midrule
    $\cft=\tfrac{1}{D}\sum_d p_d^d$ & Average continual fine-tuning performance \\ \midrule
    $\lc=\tfrac{1}{D}\sum_d p_d^D$ & Average performance of the last checkpoint \\ \midrule
    $\B_{\leftarrow n}=\tfrac{1}{D-n}\sum_{d=n}^D p_{d-n}^d$ & Average performance when a checkpoint is transferred $n$ tasks backward \\ \midrule
    $\F_{\rightarrow n}=\tfrac{1}{D-n}\sum_{d=0}^{D-n} p_{d+n}^{d}$ & Average performance when a checkpoint is transferred $n$ tasks forward \\
    \bottomrule
    \end{tabular}
\end{table}


\paragraph{Models} 
We benchmark continual learning of existing pre-trained LLMs with different architectures and sizes.
In particular, we consider \textit{(i)} encoder-decoder models (\robertab and \robertal) trained on Wikipedia \citep{liu2020roberta} as well as \textit{(ii)} decoder-only models (\gpts, \gptm, \gptl and \gptxl) trained on WebText \citep{radford2019language}. 


\paragraph{Dataset details} 
Our continual pre-training dataset is a subset of the Massively Multi-Domain Dataset (M2D2) \cite{reid2022m2d2}, which is a fine-grained, massively multi-domain corpus originally introduced for studying domain adaptation. It consists of 8.5B tokens extracted from Wikipedia and Semantic Scholar, referred to as Wikipedia and S2ORC portions. For computational concerns, we \caca{randomly?} curate a training set of 166 finer-grained ``L2 domains'', which are grouped into 20 coarser ``L1 domains''.  In order to investigate how the order of training domains impacts our domain-incremental continual learning setup, we order the training domains based on conceptual similarity and also randomly, which we refer to as \emph{similar-order} and \emph{random-order} here on-wards.

Figure~\ref{fig:dom-sim} summarizes the important characteristics of the dataset. On the left panel is the embedding similarity matrix \caca{(right, beyza?)} in similar-order, where the two blocks along the diagonal correspond to different portions. The upper right panel shows the TSNE embeddings of all coarser domains. Likewise, we notice that Wiki domains are concentrated at the bottom right of the embedding space. Finally, the lower right panel shows the number of finer-grained L2 domains and the length of the training set for each L1 domain. As noticed, training set properties differ across domains, which we intentionally did not uniform to simulate more challenging real-world training settings. 

\paragraph{Measured quantities} Since we would like to analyze the merits of continual learning, we establish two baselines: \emph{zero-shot} perplexity of the original models and perplexity of the models \emph{fine-tuned} on each domain separately, denoted respectively by ZS and FT. While the former serves as a sanity check, exceeding the latter is the first goal set for a continual learner. To quantify continual learning performance, we compute \emph{continual fine-tuning} perplexity (CFT), obtained by testing a model on the most recent training domain. Moreover, we test the \emph{last checkpoint} (LC) on all training domains to study transfer at its most extreme. Finally, we evaluate checkpoints on old/unseen domains to measure backward/forward transfer. $\B_{\leftarrow n}$ and $\F_{\leftarrow n}$ denote $n$-task backward and forward perplexity, respectively.



==> __findings.tex <==

\section{Findings}
This section presents the main findings of our work. We begin by contrasting the continual fine-tuning and last checkpoint performance against zero-shot and standard fine-tuning. Next, we explore the forward transferability of the GPT model family to new L1 and L2 domains. Finally, we study the backward transfer.

\subsection{Analysis of continual fine-tuning and the last checkpoint}

\paragraph{Final checkpoint achieves better perplexity than zero-shot}
Our findings consistently show that, regardless of the data sequence, model family, or size, the perplexity at the final checkpoint either surpasses or equals the zero-shot performance. We report the average perplexity over all domains, suggesting that the model successfully accumulates knowledge without significantly forgetting previous domains.  Notably, randomizing the training sequence results in a more favorable average perplexity than a similar order sequence. We present a detailed comparison of perplexity values for Wiki and S2ORC datasets in Table~\ref{tab:res2}, highlighting the GPT family's tendency to forget the earlier portion while showing increased perplexity on the latter portion.
 

\input{results_main_table}

\paragraph{CFT is more favorable to standard FT when data is ordered} 
Comparing the FT column against CFT-S and CFT-R reveals that continual fine-tuning outperforms standard fine-tuning only if subsequent training domains have high similarity. This observation aligns with the premise that a model's performance on a current task is intrinsically linked to its starting checkpoint. Meaning, when training domains are ordered by similarity, the last checkpoint naturally transfers better to the next task compared to the original model. Nevertheless, in scenarios where training domains are mixed, starting from the original model proves to be more beneficial, a finding that resonates with recent research in continual test-time adaptation \citep{press2023rdumb} and checkpoint selection strategies for language models \citep{fisch2023towards}.

\paragraph{Improvement correlates with model size}
In agreement with the recent literature on scaling laws, continual learning of bigger models results in better CFT and LC performance irrespective of the training order. However, this consistent pattern cannot solely be attributed to continual learning since zero-shot performance is heavily influenced by model size. We thus take the zero-shot performance as a baseline and analyze how much CFT and LC perplexities improve over zero-shot. We observe a clear inverse correlation between the gain and model size, e.g., the smallest model benefits the most from continual learning. 

\paragraph{Forgetting in \roberta family is not evident} 
In contrast to the GPT family, our analysis reveals that the \roberta family does not exhibit forgetting of old tasks during continual training. This indicates that gradient descent updates do not interfere with old tasks. To illustrate this, we present a visualization of backward transfer performance across four randomly selected domains in Figure~\ref{fig:backward-one-domain-roberta}. Similar findings with encoder-decoder models were reported in \citep{cossu2022continual}. We conjecture that modifying the model architecture by including a bottleneck layer plays a significant role in this behavior.

\paragraph{Generalization may deteriorate due to continual learning}
As indicated in Table~\ref{tab:res2}, while fine-tuning on Wiki domains shows minimal improvement, a significant increase is observed in the S2ORC domains. To decipher this, we visualize fine-tuning traces on four randomly chosen domains in Figure~\ref{fig:tr-path}. For all model sizes, as expected, the training and test losses on S2ORC domains steadily decrease. Surprisingly, the loss computed on the validation and test sets, as well as on the first three percent of the training set, increases during optimization (note that increasing model capacity seems to help with this degradation). This counter-intuitive observation suggests that the original models, pre-trained on extensive, high-quality datasets, possess better generalization capabilities than those fine-tuned on specific Wiki portions. \caca{word overlap between WebText and Wiki/S2ORC}.

\begin{figure}[t]
    \centering
    \includegraphics[width=.99\linewidth]{figs/forward/gpt2-short.png} % \\
    % \includegraphics[width=.99\linewidth]{figs/forward/roberta-short.png}
    \caption{Forward transfer results with similar training order. The checkpoints are saved after training on an L1 domain ends. Each panel shows the forward performance on one domain (stated in the title), which is obtained by evaluating all previous checkpoints on that domain. The dashed lines show zero-shot performance. $x$ and $y$ axes correspond to L1 domain ids and perplexities, respectively. The grey background highlights Wiki domains. See Figure~\ref{fig:forw-L1-long} for the complete results. \caca{discussion'a qa yapamadigimizi, ama idealin bu oldugunu ekle}}
    \label{fig:forw-L1}
\end{figure}

\begin{figure}[t]
    \centering
    \includegraphics[width=.99\linewidth]{figs/forward/avg-forw.png}
    \caption{Forward transfer results with random similar training order. Unlike Figure~\ref{fig:forw-L1}, we checkpoint after each L2 domain (hence 165 checkpoints). The $x$ axis shows the number of domains on which the model is trained before being transferred and the curves denote the change in perplexity (normalized by zero-shot). We observe clear positive/negative forward transfer to S2ORC/Wiki portions. Also, the declining purple curve suggests knowledge accumulation.}
    \label{fig:forw-L2}
\end{figure}

\subsection{Forward transfer}
Next, we investigate to what extent forward transfer is possible.
Figure~\ref{fig:forw-L1} demonstrates the first set of results, where we transfer checkpoints trained in similar order to future L1 domains (see Figure~\ref{fig:forw-L1-long} for complete results).
To aid the visual inspection, we plot the decoder-only and encoder-decoder models separately and explain these findings in the next two paragraphs.
For a finer-grained analysis, we forward transfer all checkpoints to future L2 domains (random training order).
Due to the heavy computational burden (a total of 13.695 evaluations), we performed this analysis only with \gpts checkpoints.

\paragraph{Decoder-only models rarely transfer well} 
\textit{(i)} Most notably, pre-training on a handful of domains leads to significantly worse forward transfer performance compared to zero-shot (the dotted horizontal lines).
In contrast, long enough pre-training on different domains sometimes leads to positive forward transfer (panels 13-14).
\textit{(ii)} We  notice a \textit{recency effect} in that the forward transfer performance increases if the test domain and the most recent training domain belong to the same training portion, which is most visible in panels 13 and 19:
After switching from Wikipedia to the S2ORC portion at the ninth L1 domain, the performance on the unseen ``math articles'' domain remarkably increases. 
As expected, we observe the opposite effect in panel 19, where the test performance on the ``natural and physical sciences'' domain, which belongs to the Wikipedia portion, dramatically degrades with a change in the training portion.
\textit{(iii)} Finally, we observe that forward transfer perplexity correlates with model size.

\paragraph{Encoder-decoder models require just a few L1 domains for good transfer}
\textit{(i)} In stark contrast with the decoder-only models, pre-training even on the first L1 domain helps to exceed zero-shot performance (comparing the dotted lines and the first point of each sequence). Interestingly, this holds when the pre-training and test domains belong to different portions of the training set.
\textit{(ii)} We further notice the forward transfer perplexity tends to improve for the first ten L1 domains and later slightly degrade. Since it is still considerably above zero-shot performance, we chose not to investigate this in detail.
\textit{(iii)} Lastly, the model size does not seem to influence forward transfer performance, which is again as opposed to decoder-only models.


\paragraph{Random-order training enables positive transfer to S2ORC} 
As noted earlier, we test every checkpoint on all future L2 domains and consider random training order. 
Unlike the recently presented results, this time 
Figure~\ref{fig:forw-L2} illustrates the improvement in the perplexity (relative to zero-shot) as a function of the number of continual pre-training domains prior to forward transfer. 
\textit{(i)} Noticeably, positive forward transfer is possible only to the S2ORC portion since all values corresponding to the Wikipedia test portion are positive, implying no perplexity improvement when tested on the Wikipedia portion. 
We find this finding rather intuitive as the S2ORC portion is much bigger than the Wiki portion. 
Consequently, when the model is transferred to domains from which not much training data has been seen, test performance quickly degrades.
% This finding aligns well with the previous observation that fine-tuning on certain Wikipedia domains causes worse generalization. 
\textit{(ii)} Further, test perplexity on the S2ORC portion shows a clear positive correlation with the number of pre-training tasks, i.e., longer training before transfer improves transfer perplexity.
We conclude that the model accumulates knowledge that is on average beneficial to predict next tokens.

\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{figs/ablations/train-pathology-gpt2-small.png}
    \caption{For GPT models with different sizes and four domains, we visualize the training loss (single blue curve) as well as the loss computed on the validation test, test sets, and the first three percent of the training set.}
    \label{fig:tr-path}
\end{figure}

\subsection{Backward transfer}
Our main backward transfer findings are demonstrated in Figure~\ref{fig:backward}. We observe clearly different transfer perplexities with two training orders, which we elaborate in the next two paragraphs. Further, we randomly choose four domains and visualize the backward transfer perplexity to these domains during the course of learning, please see Figures~\ref{fig:backward-one-domain-roberta} and \ref{fig:backward-one-domain-gpt2l} for results obtained with \robertal and \gptl.

\paragraph{Similar training order facilitates backward transfer to short distances}
The left panel in Figure~\ref{fig:backward} demonstrates to what extent checkpoints transfer to older training domains when subsequent domains have high conceptual overlap. In particular, $x$-axis shows how many tasks have passed between the checkpoint and the test domain. As before, we normalize the test perplexities by respective zero-shot perplexities obtained on the same domains. The results reveal that continual learning improves the zero-shot perplexity when checkpoints are transferred up to 25-30 domains backward. Naturally, the improvement worsens over time as the recent training and test domains become more dissimilar.  We also notice that the smallest GPT model benefits as well as deteriorates the most.

\paragraph{Random training order leads to positive backward transfer}
The right panel in Figure~\ref{fig:backward} reflects a rather surprising finding that when the training domains are shuffled, we observe positive backward transfer (with respect to zero-shot performance). 
This observation holds for all members of the GPT family and for all transfer distances. For control, we prepend each curve in Figure~\ref{fig:backward} with fine-tuning performance, where we observe the most efficient transfer. Most strikingly and unlike the previous set of findings, the perplexity improvement steadily increases when we transfer to more into the past. We interpret this finding as yet another indicator for knowledge accumulation, i.e., performance on old domains increases on average when the model is trained on a mixed set of domains, only a handful of which are conceptually similar.

\begin{figure}[t]
    \centering
    \includegraphics[width=.49\linewidth]{figs/backward/avg-backw-all-similar.png}
    \includegraphics[width=.49\linewidth]{figs/backward/avg-backw-all-random.png}
    \includegraphics[width=.99\linewidth]{figs/backward/avg-backw-stages-all-random.png}
    \caption{Average backward transfer performance as a function of the number of tasks between the checkpoint and the tested domain. The first points in each curve correspond to continual fine-tuning (no backward transfer), which serves as an upper bound on the backward transfer. The benefits of continual learning when trained in similar order steadily degrade by the transfer distance while we observe the opposite in random order training. \caca{discuss below fig}}
    \label{fig:backward}
\end{figure}


\paragraph{\robertal always exhibits positive backward transfer while \gptl transfer performance depends heavily on the transferred domain}
Looking into Figure~\ref{fig:backward-one-domain-roberta}, we notice that backward transfer perplexity of \robertal remains relatively close to fine-tuning performance. Interestingly, we observe occasional jumps in perplexity when trained in random order, whose analysis is an interesting future work. On the other hand, Figure~\ref{fig:backward-one-domain-gpt2l} demonstrates backward transfer to the same four domains when \gptl is trained. In agreement with our earlier findings, switching from Wiki portion to S2ORC causes a significant perplexity degradation on Wiki domains when trained in similar order. Further, the characteristics of the test domain seem to determine whether the transfer is positive or negative. Finally, we observe a less fluctuating backward perplexity with random training order.


% \subsection{General forgetting}


\subsection{Ablation studies}

\paragraph{Batch size impacts the learning when trained in similar order} As an ablation study, we increase the batch size from 16 to 64, thereby a quarter of gradient updates. Figure~\ref{fig:small64} compares the results of different batch sizes. When trained in random order, continual fine-tuning and last checkpoint performances virtually remain the same despite varying the batch size. In similar training order, a smaller batch size helps improve continual fine-tuning perplexity but worsens the performance of the last checkpoint. As before, we conjecture that taking more gradient steps aids the model to better fit the current task while leading to forgetting of the old tasks.

\paragraph{Balanced the data size across L2 domains does not improve performance} Next, we investigate whether the imbalance in training data sizes impacts the overall performance (see Figure~\ref{fig:dom-sim} for L1 domain lengths \caca{[what is length here?]}). For this, we equalize the number of data points for all L2 domains and train from scratch, which requires cropping several domains' data. Figure~\ref{fig:balanced} shows the resulting continual fine-tuning and last checkpoint perplexities. For both metrics, test performance on almost all L2 domains deteriorates after balancing the domain sizes. Consequently, the results suggest using all data at hand instead of leaving some out for the sake of balance.

\paragraph{Swapping Wiki and S2ORC portions causes more uniform perplexity} Finally, we swap the portions for similar order training, i.e., start the training with S2ORC, followed by the Wiki portion. Arguably, such a training order still follows conceptual similarity; hence, it allows us to see whether our previous findings generalize. The left panel in Figure~\ref{fig:reversed} shows that the continual fine-tuning perplexity remains almost the same. However, the last checkpoint perplexity significantly changes (see the right panel). While the performance on the S2ORC portion significantly degrades, we observe the opposite effect for the Wiki portion. Agreeing with our previous findings, we conclude that the last checkpoint performs worse when tested on older domains.

% \section{How to mitigate forgetting}
% \paragraph{Weight averaging}
% We take two checkpoints trained lastly on domains $i$ and $j$. 
% We linearly average the weights $\theta \leftarrow \lambda \theta_i + (1-\lambda)\theta_j$, and test the resulting networks $\lambda \in \{0,0.1,\ldots,1.0\}$ on domains $i$ and $j$.




==> ablation_lr.tex <==
\begin{figure}[h]
	\centering
	\caption{Difficult to explain hyper-parameter ablation results. Both results are obtained with \gpts. \caca{[include training and testing loss plots]}}
	\label{fig:hyperpars}
	\includegraphics[width=.9\linewidth]{figs/ablations/hyper-1.png}
	\includegraphics[width=.9\linewidth]{figs/ablations/hyper-2.png}
\end{figure}


==> results_main_table_delete.tex <==

% \begin{table*}
%     \centering
%     \begin{tabular}{l||c|c|c||c|c||c|c} 
%         \toprule
%         % \multicolumn{7}{c}{\textsc{Perplexity computed on all domains}} \\
%         % \toprule
%         \multicolumn{4}{c||}{} & \multicolumn{2}{c||}{\textsc{\simi}} &  \multicolumn{2}{c}{\textsc{\rand}} \\
%          \midrule
%          & Num. & Zero & Pre- & Continual & Last & Continual & Last \\
%          & pars. & shot & training & pretraining & checkpoint & pretraining & checkpoint \\
%          % & & (ZS) & (PT) & (CFT-S) & (LC-S) & (CFT-R) & (LC-R) \\
%          \midrule
%          \textcolor{gpts}{\textbf{\gpts}} & 117M & 27.90  & 20.36 {\scriptsize \textbf{(-7.54)}}  & 19.46 {\scriptsize \textbf{(-8.44)}}  & 27.52 {\scriptsize \textbf{(-0.38)}}  & 21.04 {\scriptsize \textbf{(-6.86)}}  & 22.47 {\scriptsize \textbf{(-5.43)}}  \\
%          \midrule
%          \textcolor{gptm}{\textbf{\gptm}} & 345M & 21.54  & 18.58 {\scriptsize \textbf{(-2.96)}}  & 16.58 {\scriptsize \textbf{(-4.96)}}  & 20.11 {\scriptsize \textbf{(-1.43)}}  & 16.84 {\scriptsize \textbf{(-4.7)}}  & 19.01 {\scriptsize \textbf{(-2.53)}} \\
%          \midrule
%          \textcolor{gptl}{\textbf{\gptl}} & 774M & 18.89  & 14.43 {\scriptsize \textbf{(-4.46)}}  & 14.33 {\scriptsize \textbf{(-4.56)}}  & 18.68 {\scriptsize \textbf{(-0.21)}}  & 15.13 {\scriptsize \textbf{(-3.76)}}  & 17.19 {\scriptsize \textbf{(-1.7)}} \\
%          \midrule
%          \textcolor{gptxl}{\textbf{\gptxl}} & 1.5B & 17.36  & 12.43 {\scriptsize \textbf{(-4.93)}}  & 12.28 {\scriptsize \textbf{(-5.08)}}  & 15.29 {\scriptsize \textbf{(-2.07)}}  & 13.89 {\scriptsize \textbf{(-3.47)}}  & 15.24 {\scriptsize \textbf{(-2.12)}}  \\ 
%          \midrule
%          \midrule
%          \textcolor{llama}{\textbf{\llama}} & 7B & 6.87  & 23.5  & 8.54  & 14.86  & 10.09 & 12.02   \\ 
%          \bottomrule
%     \end{tabular}
%     \caption{\label{tab:res} This table shows test perplexities ($\downarrow$) with different model sizes and training orders. For reference, we include the zero-shot and fine-tuning perplexities. Please see Table~\ref{tab:res2} for results obtained on Wiki and S2ORC domains. Inside the parentheses are the perplexity improvements over zero-shot (the smaller the better).}
% \end{table*}


\begin{table*}
    \centering
    \caption{This table shows test perplexities ($\downarrow$) with different model sizes and training orders. For reference, we include the zero-shot and fine-tuning perplexities. Please see Table~\ref{tab:res2} for results obtained on Wiki and S2ORC domains. Inside the parentheses are the perplexity improvements over zero-shot (the smaller the better).}
    \label{tab:res} 
    \begin{tabular}{l||c|c||c|c||c|c} 
        \toprule
        % \multicolumn{7}{c}{\textsc{Perplexity computed on all domains}} \\
        % \toprule
        \multicolumn{3}{c||}{} & \multicolumn{2}{c||}{\textsc{\simi}} &  \multicolumn{2}{c}{\textsc{\rand}} \\
         \midrule
         & Zero & Dom. adapt. & Continual & Last & Continual & Last \\
         & shot & pretraining & pretraining & checkpoint & pretraining & checkpoint \\
         % & & (ZS) & (PT) & (CFT-S) & (LC-S) & (CFT-R) & (LC-R) \\
         \midrule

\textcolor{gpts}{\textbf{\gpts}} &	28.35 &	21.48\scriptsize{\textbf{(-6.87)}} &	19.38\scriptsize{\textbf{(-8.97)}} &	24.79\scriptsize{\textbf{(-3.56)}} &	19.67\scriptsize{\textbf{(-8.68)}} &	20.50\scriptsize{\textbf{(-7.85)}} \\ \midrule
\textcolor{gptm}{\textbf{\gptm}} &	21.78 &	19.73\scriptsize{\textbf{(-2.05)}} & 16.69\scriptsize{\textbf{(-5.09)}} &	19.33\scriptsize{\textbf{(-2.45)}} &	15.74\scriptsize{\textbf{(-6.04)}} &	16.82\scriptsize{\textbf{(-4.96)}} \\ \midrule
\textcolor{gptl}{\textbf{\gptl}} &	19.20 &	15.27\scriptsize{\textbf{(-3.92)}} &	14.30\scriptsize{\textbf{(-4.90)}} &	17.14\scriptsize{\textbf{(-2.06)}} &	14.40\scriptsize{\textbf{(-4.79)}} &	15.42\scriptsize{\textbf{(-3.78)}} \\ \midrule
\textcolor{gptxl}{\textbf{\gptxl}} &	17.68 &	13.28\scriptsize{\textbf{(-4.40)}} &	12.03\scriptsize{\textbf{(-5.65)}} &	13.63\scriptsize{\textbf{(-4.05)}} &	13.22\scriptsize{\textbf{(-4.46)}} &	13.72\scriptsize{\textbf{(-3.96)}} \\ \midrule\midrule
\textcolor{llama}{\textbf{\llama}} &	 6.84 &	11.32\scriptsize{\textbf{(4.48)}} &	 8.42\scriptsize{\textbf{(1.58)}} &	11.42\scriptsize{\textbf{(4.58)}} &	 9.06\scriptsize{\textbf{(2.22)}} &	11.54\scriptsize{\textbf{(4.69)}} \\
         \bottomrule
    \end{tabular}
\end{table*}

==> results_main_table_portions.tex <==

% \begin{table*}[h]
%     \centering
%     \caption{A more detailed analysis of our main results table. This time, we compute the test perplexities($\downarrow$) on Wiki and S2ORC portions separately.}
%     \label{tab:res2} 
%     \begin{tabular}{c|l||c|c||c|c|c||c|c|c} 
%         \toprule
%         \multicolumn{4}{c||}{} & \multicolumn{3}{c||}{\textsc{\simi}} &  \multicolumn{3}{c}{\textsc{\rand}} \\
%          \midrule
%          Test & \multirow{2}{*}{Model} & Zero & Dom. adapt. & Continual & Final &   \multirow{2}{*}{Forg.} & Continual & Final &  \multirow{2}{*}{Forg.} \\
%          portion & & shot & pretraining & pretraining & model & & pretraining & model & \\
%          \cmidrule{1-10}
%          \multirow{5}{*}{Wiki} & \textcolor{gpts}{\textbf{\gpts}} & 26.69 &	25.42\scriptsize{\textbf{(-1.27)}} &	30.15\scriptsize{\textbf{( 3.46)}} &	46.41\scriptsize{\textbf{(19.72)}} & 0.37 &	34.11\scriptsize{\textbf{( 7.42)}} &	37.51\scriptsize{\textbf{(10.82)}}   & 2.17 \\
%          \cmidrule{2-10}
%          & \textcolor{gptm}{\textbf{\gptm}} & 20.42 &	23.34\scriptsize{\textbf{( 2.92)}} &	23.76\scriptsize{\textbf{( 3.34)}} & 	29.29\scriptsize{\textbf{( 8.87)}} &	0.66 & 26.47\scriptsize{\textbf{( 6.05)}} &	32.14\scriptsize{\textbf{(11.72)}}  & 2.10 \\
%          \cmidrule{2-10}
%          & \textcolor{gptl}{\textbf{\gptl}} & 17.80 &	17.40\scriptsize{\textbf{(-0.41)}} &	20.63\scriptsize{\textbf{( 2.83)}} & 	30.12\scriptsize{\textbf{(12.32)}}  &	0.99 & 23.28\scriptsize{\textbf{( 5.48)}} &	28.99\scriptsize{\textbf{(11.19)}}  & 1.91 \\
%          \cmidrule{2-10}
%          & \textcolor{gptxl}{\textbf{\gptxl}} & 16.31 &	15.23\scriptsize{\textbf{(-1.08)}} &	18.75\scriptsize{\textbf{( 2.44)}} &	26.07\scriptsize{\textbf{( 9.76)}} & 0.71 &	21.57\scriptsize{\textbf{( 5.27)}} &	25.32\scriptsize{\textbf{( 9.01)}}  & 1.39 \\
%          \cmidrule{2-10}
%          & \textcolor{llama}{\textbf{Llama2}} & 5.83 &	21.02\scriptsize{\textbf{(15.19)}} &	 9.40\scriptsize{\textbf{( 3.57)}} &	11.58\scriptsize{\textbf{( 5.75)}} & 0.15 &	17.42\scriptsize{\textbf{(11.59)}} &	11.70\scriptsize{\textbf{( 5.87)}} & 1.38 \\
%          \midrule
%          \midrule
%          \multirow{5}{*}{S2ORC} & \textcolor{gpts}{\textbf{\gpts}} & 28.83 &	19.99\scriptsize{\textbf{(-8.84)}} &	16.70\scriptsize{\textbf{(-12.13)}} &	22.98\scriptsize{\textbf{(-5.85)}} & 6.59 &	17.76\scriptsize{\textbf{(-11.07)}} &	19.29\scriptsize{\textbf{(-9.54)}}  & 1.74 \\
%          \cmidrule{2-10}
%          & \textcolor{gptm}{\textbf{\gptm}} &22.34 &	18.35\scriptsize{\textbf{(-3.99)}} &	14.95\scriptsize{\textbf{(-7.40)}} &	18.42\scriptsize{\textbf{(-3.92)}} & 2.55 &	14.41\scriptsize{\textbf{(-7.93)}} &	15.77\scriptsize{\textbf{(-6.57)}} & 1.66 \\
%          \cmidrule{2-10}
%          & \textcolor{gptl}{\textbf{\gptl}} & 19.64 &	14.26\scriptsize{\textbf{(-5.38)}} &	13.00\scriptsize{\textbf{(-6.64)}} &	16.05\scriptsize{\textbf{(-3.59)}} & 3.44 &	13.12\scriptsize{\textbf{(-6.52)}} &	14.31\scriptsize{\textbf{(-5.33)}}   & 1.48 \\
%          \cmidrule{2-10}
%          & \textcolor{gptxl}{\textbf{\gptxl}} & 18.08 &	12.10\scriptsize{\textbf{(-5.99)}} &	10.64\scriptsize{\textbf{(-7.44)}} &	12.85\scriptsize{\textbf{(-5.24)}} & 2.43 &	11.74\scriptsize{\textbf{(-6.35)}} &	12.28\scriptsize{\textbf{(-5.81)}} & 1.29  \\ 
%          \cmidrule{2-10}
%          & \textcolor{llama}{\textbf{Llama2}} & 6.93 &	10.58\scriptsize{\textbf{( 3.65)}} &	 7.99\scriptsize{\textbf{( 1.06)}} & 	11.58\scriptsize{\textbf{( 4.65)}} &	2.3 & 9.58\scriptsize{\textbf{( 2.65)}} &	11.70\scriptsize{\textbf{( 4.77)}} & 1.2  \\
%          \bottomrule
%     \end{tabular}
% \end{table*}

==> results_main_table_tmlr.tex <==
% \begin{table*}
%     \centering
%     \caption{This table shows test perplexities ($\downarrow$) with different model sizes and training orders. For reference, we include the zero-shot and fine-tuning perplexities. Please see Table~\ref{tab:res2} for results obtained on Wiki and S2ORC domains. Inside the parentheses are the perplexity improvements over zero-shot (the smaller the better).}
%     \label{tab:res} 
%     \begin{tabular}{l||c|c||c|c|c||c|c|c} 
%         \toprule
%         % \multicolumn{7}{c}{\textsc{Perplexity computed on all domains}} \\
%         % \toprule
%         \multicolumn{3}{c||}{} & \multicolumn{3}{c||}{\textsc{\simi}} &  \multicolumn{3}{c}{\textsc{\rand}} \\
%          \midrule
%          & Zero & Dom. adapt. & Continual & Last & \multirow{2}{*}{Forg.} & Continual & Last & \multirow{2}{*}{Forg.} \\
%          & shot & pretraining & pretraining & checkpoint & & pretraining & checkpoint & \\
%          % & & (ZS) & (PT) & (CFT-S) & (LC-S) & (CFT-R) & (LC-R) \\
%          \midrule

% \textcolor{gpts}{\textbf{\gpts}} &	28.35 &	21.48\scriptsize{\textbf{(-6.87)}} &	19.38\scriptsize{\textbf{(-8.97)}} &	24.79\scriptsize{\textbf{(-3.56)}} & 5.63	 &	19.67\scriptsize{\textbf{(-8.68)}} &	20.50\scriptsize{\textbf{(-7.85)}} & 1.87 \\ \midrule
% \textcolor{gptm}{\textbf{\gptm}} &	21.78 &	19.73\scriptsize{\textbf{(-2.05)}} & 16.69\scriptsize{\textbf{(-5.09)}} &	19.33\scriptsize{\textbf{(-2.45)}} & 2.33	& 15.74\scriptsize{\textbf{(-6.04)}} &	16.82\scriptsize{\textbf{(-4.96)}} & 1.78 \\ \midrule
% \textcolor{gptl}{\textbf{\gptl}} &	19.20 &	15.27\scriptsize{\textbf{(-3.92)}} &	14.30\scriptsize{\textbf{(-4.90)}} &	17.14\scriptsize{\textbf{(-2.06)}} & 2.91 	& 14.40\scriptsize{\textbf{(-4.79)}} &	15.42\scriptsize{\textbf{(-3.78)}} & 1.55 \\ \midrule
% \textcolor{gptxl}{\textbf{\gptxl}} &	17.68 &	13.28\scriptsize{\textbf{(-4.40)}} &	12.03\scriptsize{\textbf{(-5.65)}} &	13.63\scriptsize{\textbf{(-4.05)}} & 1.89	& 13.22\scriptsize{\textbf{(-4.46)}} &	13.72\scriptsize{\textbf{(-3.96)}} & 1.32 \\ \midrule\midrule
% \textcolor{llama}{\textbf{\llama}} &	 6.84 &	11.32\scriptsize{\textbf{(4.48)}} &	 8.42\scriptsize{\textbf{(1.58)}} &	11.42\scriptsize{\textbf{(4.58)}} & 1.31	 & 9.06\scriptsize{\textbf{(2.22)}} &	11.54\scriptsize{\textbf{(4.69)}} & 1.24 \\
%          \bottomrule
%     \end{tabular}
% \end{table*}



==> results_roberta_table_portions.tex <==

% \begin{table*}[t]
%     \centering
%     \begin{tabular}{c|l||c|c||c|c||c|c}  
%         \toprule
%         \multicolumn{4}{c||}{} & \multicolumn{2}{c||}{\textsc{\simi}} &  \multicolumn{2}{c}{\textsc{\rand}} \\
%          \midrule
%          Test & \multirow{2}{*}{Model} & Zero & Pre- & Continual & Final & Continual & Final \\
%          portion & & shot & training & pretraining & model & pretraining & model \\
%          \midrule
%          \multirow{2}{*}{All} & \robertab & 1.97  &  1.73  &  1.54  &  1.46  &  1.27  &  1.26 \\
%          \cmidrule{2-8}
%          & \robertal & 4.98  &  3.10  &  2.43  &  2.34  &  1.37  &  1.28 \\
%          \midrule
%          \midrule
%          \multirow{2}{*}{Wiki} & \robertab & 1.93  &  1.69  &  1.49  &  1.43  &  1.45  &  1.48 \\
%          \cmidrule{2-8}
%          & \robertal & 4.73  &  2.95  &  2.38  &  2.32  &  1.61  &  1.54 \\
%          \midrule
%          \midrule
%          \multirow{2}{*}{S2ORC} & \robertab & 1.56  &  1.37  &  1.26  &  1.26  &  1.25  &  1.26 \\
%          \cmidrule{2-8}
%          & \robertal & 2.56  &  1.61  &  2.15  &  2.15  &  1.35  &  1.29 \\
%          \bottomrule
%     \end{tabular}
%     \caption{\label{tab:roberta} Test perplexities obtained with \roberta family.}
% \end{table*}


